PETformer: Long-term Time Series Forecasting via Placeholder-enhanced Transformer

Recently, the superiority of Transformer for long-term time series forecasting (LTSF) tasks has been challenged, particularly since recent work has shown that simple models can outperform numerous Transformer-based approaches. This suggests that a notable gap remains in fully leveraging the potential of Transformer in LTSF tasks. Consequently, this study investigates key issues when applying Transformer to LTSF, encompassing aspects of temporal continuity, information density, and multi-channel relationships. We introduce the Placeholder-enhanced Technique (PET) to enhance the computational efficiency and predictive accuracy of Transformer in LTSF tasks. Furthermore, we delve into the impact of larger patch strategies and channel interaction strategies on Transformer's performance, specifically Long Sub-sequence Division (LSD) and Multi-channel Separation and Interaction (MSI). These strategies collectively constitute a novel model termed PETformer. Extensive experiments have demonstrated that PETformer achieves state-of-the-art performance on eight commonly used public datasets for LTSF, surpassing all existing models. The insights and enhancement methodologies presented in this paper serve as valuable reference points and sources of inspiration for future research endeavors.

==> tables/ablation_channel.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[htb]
\centering
\caption{Ablation study of the MSI. The direct channel mixing (DCM) approach is compared with the MSI approach. For the MSI method, various strategies illustrated in Figure \ref{fig4} are evaluated.}
\label{ablation_channel}
\begin{adjustbox}{max width=0.75\linewidth}
\begin{tabular}{@{}ccllcccccccc@{}}
\toprule
\multicolumn{2}{c}{Models}                                               & \multicolumn{2}{c}{DCM}                               & \multicolumn{2}{c}{MSI/NCI}                & \multicolumn{2}{c}{MSI/SA}                 & \multicolumn{2}{c}{MSI/CI}      & \multicolumn{2}{c}{MSI/CA}      \\ \midrule
\multicolumn{2}{c}{Metric}                                               & \multicolumn{1}{c}{MSE}   & \multicolumn{1}{c}{MAE}   & MSE                       & MAE            & MSE            & MAE                       & MSE            & MAE            & MSE            & MAE            \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{ETTh1}}   & \multicolumn{1}{c|}{96}  & \multicolumn{1}{c}{0.409} & \multicolumn{1}{c}{0.435} & {\ul 0.348}               & 0.379          & \textbf{0.348} & 0.379                     & 0.349          & {\ul 0.378}    & 0.349          & \textbf{0.378} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & \multicolumn{1}{c}{0.470} & \multicolumn{1}{c}{0.476} & {\ul 0.389}               & {\ul 0.403}    & \textbf{0.389} & \textbf{0.403}            & 0.394          & 0.407          & 0.393          & 0.407          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{336} & \multicolumn{1}{c}{0.512} & \multicolumn{1}{c}{0.503} & {\ul 0.419}               & {\ul 0.419}    & 0.419          & 0.420                     & \textbf{0.415} & \textbf{0.417} & 0.426          & 0.426          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{720} & \multicolumn{1}{c}{0.626} & \multicolumn{1}{c}{0.574} & {\ul 0.444}               & {\ul 0.452}    & \textbf{0.435} & \textbf{0.447}            & 0.454          & 0.458          & 0.453          & 0.461          \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Weather}} & \multicolumn{1}{c|}{96}  & 0.147                     & 0.195                     & {\ul 0.145}               & 0.185          & 0.145          & \textbf{0.184}            & 0.145          & 0.185          & \textbf{0.144} & {\ul 0.184}    \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 0.198                     & 0.245                     & \multicolumn{1}{l}{0.189} & \textbf{0.228} & 0.189          & {\ul 0.228}               & \textbf{0.188} & 0.229          & {\ul 0.189}    & 0.228          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{336} & 0.255                     & 0.291                     & \multicolumn{1}{l}{0.241} & \textbf{0.270} & {\ul 0.241}    & {\ul 0.270}               & 0.242          & 0.272          & \textbf{0.241} & 0.271          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{720} & 0.321                     & 0.340                     & \multicolumn{1}{l}{0.315} & 0.323          & {\ul 0.313}    & {\ul 0.322}               & \textbf{0.311} & \textbf{0.322} & 0.314          & 0.324          \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Traffic}} & \multicolumn{1}{c|}{96}  & 1.530                     & 0.621                     & \textbf{0.357}            & \textbf{0.240} & 0.363          & \multicolumn{1}{l}{0.249} & {\ul 0.359}    & {\ul 0.243}    & 0.365          & 0.248          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 1.516                     & 0.614                     & {\ul 0.376}               & \textbf{0.248} & 0.377          & \multicolumn{1}{l}{0.253} & \textbf{0.375} & {\ul 0.249}    & 0.386          & 0.257          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{336} & 1.546                     & 0.631                     & \textbf{0.392}            & \textbf{0.255} & 0.393          & \multicolumn{1}{l}{0.262} & {\ul 0.393}    & {\ul 0.257}    & 0.400          & 0.265          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{720} & 1.566                     & 0.644                     & \textbf{0.430}            & \textbf{0.276} & {\ul 0.430}    & \multicolumn{1}{l}{0.282} & 0.431          & {\ul 0.278}    & 0.438          & 0.285          \\ \midrule
\multicolumn{2}{c|}{\textbf{Avg.}}                                       & \multicolumn{1}{c}{0.758} & \multicolumn{1}{c}{0.464} & {\ul 0.337}               & \textbf{0.307} & \textbf{0.337} & 0.308                     & 0.338          & {\ul 0.308}    & 0.341          & 0.311          \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/ablation_granularity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htb]
\centering
\caption{Ablation study of the LSD. A comparison of performance between using single points and sub-sequences as input granularity is presented. For the LSD, various window lengths \(w \in \left \{ 6,12,24,48\right \}\) are evaluated. The '-' symbol denotes out-of-memory issues encountered in our experimental environment.}
\label{ablation_granularity}
\begin{adjustbox}{max width=0.75\linewidth}
\begin{tabular}{@{}ccccllclcccc@{}}
\toprule
\multicolumn{2}{c}{Models}                                               & \multicolumn{2}{c}{Point} & \multicolumn{2}{c}{LSD/w=6}                           & \multicolumn{2}{c}{LSD/w=12}                          & \multicolumn{2}{c}{LSD/w=24} & \multicolumn{2}{c}{LSD/w=48\(^\dagger\)}    \\ \midrule
\multicolumn{2}{c}{Metric}                                               & MSE         & MAE         & \multicolumn{1}{c}{MSE}   & \multicolumn{1}{c}{MAE}   & MSE                       & \multicolumn{1}{c}{MAE}   & MSE            & MAE         & MSE            & MAE            \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{ETTh1}}   & \multicolumn{1}{c|}{96}  & 0.910       & 0.424       & \multicolumn{1}{c}{0.435} & 0.424                     & 0.361                     & 0.390                     & {\ul 0.349}    & {\ul 0.380} & \textbf{0.347} & \textbf{0.377} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 0.920       & 0.472       & \multicolumn{1}{c}{0.517} & 0.472                     & 0.406                     & 0.416                     & {\ul 0.392}    & {\ul 0.405} & \textbf{0.390} & \textbf{0.404} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{336} & 0.815       & 0.539       & \multicolumn{1}{c}{0.636} & 0.539                     & 0.435                     & 0.430                     & {\ul 0.424}    & {\ul 0.425} & \textbf{0.419} & \textbf{0.418} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{720} & 0.832       & 0.604       & \multicolumn{1}{c}{0.719} & 0.604                     & 0.461                     & 0.468                     & {\ul 0.456}    & {\ul 0.458} & \textbf{0.437} & \textbf{0.449} \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Weather}} & \multicolumn{1}{c|}{96}  & 0.159       & 0.202       & 0.159                     & 0.200                     & \multicolumn{1}{l}{0.149} & 0.189                     & {\ul 0.146}    & {\ul 0.186} & \textbf{0.146} & \textbf{0.186} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 0.206       & 0.243       & 0.206                     & 0.244                     & \multicolumn{1}{l}{0.193} & 0.233                     & \textbf{0.189} & {\ul 0.229} & {\ul 0.190}    & \textbf{0.229} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{336} & 0.255       & 0.289       & 0.256                     & 0.284                     & \multicolumn{1}{l}{0.244} & 0.274                     & \textbf{0.241} & {\ul 0.271} & {\ul 0.241}    & \textbf{0.271} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{720} & 0.323       & 0.333       & 0.326                     & 0.340                     & \multicolumn{1}{l}{0.315} & 0.327                     & \textbf{0.312} & {\ul 0.324} & {\ul 0.314}    & \textbf{0.323} \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Traffic}} & \multicolumn{1}{c|}{96}  & -           & -           & 0.437                     & 0.316                     & 0.378                     & \multicolumn{1}{c}{0.251} & {\ul 0.365}    & {\ul 0.243} & \textbf{0.357} & \textbf{0.240} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & -           & -           & 0.485                     & 0.356                     & 0.392                     & \multicolumn{1}{c}{0.257} & {\ul 0.382}    & {\ul 0.250} & \textbf{0.376} & \textbf{0.248} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{336} & -           & -           & 0.492                     & 0.345                     & 0.413                     & \multicolumn{1}{c}{0.270} & {\ul 0.397}    & {\ul 0.258} & \textbf{0.392} & \textbf{0.255} \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{720} & -           & -           & 0.485                     & 0.327                     & 0.483                     & \multicolumn{1}{c}{0.326} & {\ul 0.435}    & {\ul 0.278} & \textbf{0.430} & \textbf{0.276} \\ \midrule
\multicolumn{2}{c|}{\textbf{Avg.}}                                       & -           & -           & \multicolumn{1}{c}{0.429} & \multicolumn{1}{c}{0.371} & 0.352                     & \multicolumn{1}{c}{0.319} & {\ul 0.341}    & {\ul 0.309} & \textbf{0.337} & \textbf{0.306} \\ \bottomrule
\\ \multicolumn{12}{l}{\(\dagger\) denotes the default mode in this work.}
\end{tabular}
\end{adjustbox}
\end{table}
